Toward Scalable Algorithms for the Unsplittable Shortest Path Routing Problem

In this paper, we consider the Delay Constrained Unsplittable Shortest Path Routing problem which arises in the field of traffic engineering for IP networks. This problem consists, given a directed graph and a set of commodities, to compute a set of routing paths and the associated administrative weights such that each commodity is routed along the unique shortest path between its origin and its destination, according to these weights. We present a compact MILP formulation for the problem, extending the work in (A. Bley, 2010) along with some valid inequalities to strengthen its linear relaxation. This formulation is used as the bulding block of an iterative approach that we develop to tackle large scale instances. We further propose a dynamic programming algorithm based on a tree decomposition of the graph. To the best of our knowledge, this is the first exact combinatorial algorithm for the problem. Finally, we assess the efficiency of our approaches through a set of experiments on state-of-the-art instances.

==> max_delay_per_instance.tex <==
Atlanta	50000
Dfn-bwin	50000
Dfn-gwin	50000
Di-yuan	1000000
France	2000
NewYork	1000000
Nobel-GER	20000
Nobel-US	100000
PDH	1000000
Polska	3000
TA1	10000000

